Error-Correcting Neural Sequence Prediction

We propose a novel neural sequence prediction method based on \textit{error-correcting output codes} that avoids exact softmax normalization and allows for a tradeoff between speed and performance. Instead of minimizing measures between the predicted probability distribution and true distribution, we use error-correcting codes to represent both predictions and outputs. Secondly, we propose multiple ways to improve accuracy and convergence rates by maximizing the separability between codes that correspond to classes proportional to word embedding similarities. Lastly, we introduce our main contribution called \textit{Latent Variable Mixture Sampling}, a technique that is used to mitigate exposure bias, which can be integrated into training latent variable-based neural sequence predictors such as ECOC. This involves mixing the latent codes of past predictions and past targets in one of two ways: (1) according to a predefined sampling schedule or (2) a differentiable sampling procedure whereby the mixing probability is learned throughout training by replacing the greedy argmax operation with a smooth approximation. ECOC-NSP leads to consistent improvements on language modelling datasets and the proposed Latent Variable mixture sampling methods are found to perform well for text generation tasks such as image captioning.

==> intro.tex <==
Beam search is often used to somewhat address this challenge by choosing to greedily search a subset of the most probable trajectories. However, for continuous state spaces generated in NLM's this is less applicable since beam search requires the use of dynamic programming over discrete states. Additionally, this is would can be costly for large vocabularies even if used with discrete state models, particularly when used at training time and can be unsuitable for state transitions that are influenced by long-term dependencies. In such cases, learning from a teacher policy with full-supervision throughout training can be sub-optimal. 

Log-likelihood has a major drawback in that incorrect predictions are treated equally wrong, leading to inefficient use of the output space. Since log-probability is only measured for the token prediction corresponding to the target, alternative incorrect predictions are treated as equally poor through normalization. Policy-gradient methods look to incorporate task-specific scores as the reward and optimize for the expected accumulated reward given predictions from the sequence model.


However, using the past targets $y_{t-n}$ and current input $x_t$ to predict $y_{t+1}$ at training time does not emulate the process at test time where the model is instead required to use its own past predictions $\hat{y}_{t-n}$ to generate the sequence. Sequence predictors can suffer from this discrepancy since they are not trained to use past predictions, which can lead to errors compounding along a generated sequence at test time. Hence, learning from high dimensional and sparsely structured patterns for conditional text generation at training time so to generate sequences from the same distribution at test time is challenging. Reinforcement learning is useful in this scenario since a model can be trained to maximize the expected accumulated reward into the future, which depends on future predictions from an arbitrary time-step.  

% on why transferring value functions is feasible for NLP
Precisely, it is easier to encode similarity of different trajectories on the sentence-level for NLP problems, than it is for RL games that may have $\geq 10^3$ turns for a single trajectory. This means it feasible to learn how similar trajectory pairs are, in a unsupervised fashion or given explicit human scores. 


Transfer learning for reinforcement learning (RL) systems is typically difficult given that the state, actions and rewards are distinctly different e.g Atari and chess. However in the context of natural language processing (NLP), many problems have similar environments (i.e vocabulary for states and actions, and rewards e.g BLEU) given the language dynamics and how humans understand language are not as different as typical RL objectives are e.g RL for robotics and games. 
\newline

==> losses.tex <==
% not included in final paper

\paragraph{Cosine Proximity Loss}

The squared cosine proximity (SCP) loss takes the cosine similarity between the last layer of the value network $V_{\Theta}$ and the last layer of the policy network $\pi_{\Theta}$. The cosine similarity is then normalized in [0, 1] using the sigmoid function. We also include this in our analysis as an alternative scoring criterion. We then optimize the RHS by using stochastic gradient descent.  

\begin{gather}\label{eq:kl_loss}
    \mathcal{L}(\theta) = 1 - \sigma\Bigg({\text{cos}}\Big(\tilde{V}^{\pi}_{\Theta}(s_t), \tilde{\pi}_{\theta}(a_t|s_t) \Big)^{2}\Bigg) \nonumber \\ 
\end{gather}

==> notation_summary.tex <==
$a \in \mathcal{A}$ = $w \in \mathcal{V}$
$y \in Y$ = tokens in target sentence
$\pi_{\theta}(a_t|s_t) \forall t \in T$ = predicted tokens
$p_{\pi_\theta}(a_t|s_t)$ probability corresponding to predicted token
$\gamma$ discount factor for distance between tokens
$s$ = reward similarity score
BP = brevity penalty
$|Y| = T$ sequence length
$\text{cos}$ = cosine similarity function
$\sigma$ = logistic function

Model terms
$V_{\phi}$ value function parameterized by $\phi$
$Q_{\omega}$ is the critic network parameterized by $\omega$

$A(s, a) = Q_{\omega}(s, a) - V(s)_{\phi}$ - acquisition function, is our action better than the average action.

$G_t$ - the expected accumulated reward onward from time t.

reference caption = target
candidate captions = prediction

==> notes/abstract.tex <==
\iffalse
Neural Sequence Prediction requires that a probability distribution is predicted as output, which involves a normalizing the decoder layer outputs with a softmax function. This can be computationally expensive as the vocabulary size that corresponds to the output dimensionality is typically very large, resulting in many exponential operations. 

This paper proposes to output binary codes that require $\mathcal{O}(\log_2(\mathcal{V}))$ computations instead of $\mathcal{O}(\mathcal{V})$ that is necessary when predicting a probability distribution. This is the first work on using error-correcting codes in language models, showing competitive performance with standard cross-entropy while resulting in a $log_2$ reduction in output dimensionality. Lastly, we show that error-correcting output codes can be used in conjunction with sampling methods that aim to mitigate the effects of \textit{exposure bias}. 
\fi

==> notes/background.tex <==
% Error-Corecting Output Codes

\iffalse
In between every power of 2, we may have some leftover bits that are used as \textit{error correcting} bits e.g $4$ bits allows for $2^{4}=16$ binary codes, if $k=10$ then we $d=6$ error correcting bits leftover which we use to separate and correct $k$ classes. 
\fi


In order to achieve good separation between $k$ classes (i.e. codewords that are assigned so that it is less likely to make mistakes due close Hamming distances), the codes should have good row and column separation. The former refers to having equidistant Hamming distances, where remaining codes are the error-correcting codes. Column separation refers to ensuring that the functions for each bit-position are uncorrelated with one another. This can be achieved by maximizing the Hamming distance between the columns, similar to row-separation. In section \autoref{sec:cc}, we will our proposed method for achieving well-separated codewords. 

\iffalse
A primary aim in ECOC is that the bit errors are uncorrelated and that likelihood of simultaneous errors occurring is low. This property makes it easier for error-correcting codes to re-correct errors. If many simultaneous errors are made, this becomes more difficult.
\iffalse
ECOCs have been used for multi-class document classification~\citep{berger1999error}. The authors also propose a coding theory argument as to why randomly assigned codes can result in well-separated codes. However, they make the strong assumption of class independence which is weak for typical natural language problems. This work addresses by using semantically-driven separation for language modelling.
\fi
ECOC can be considered an ensemble method for multi-classification where each model makes a prediction for each binary unit in $C$, albeit a distinct code that is being predicted in binary classification. ~\citet{kong1995error} have shown that this distinction over voting methods leads to variance reduction and bias-correction in each respective ECOC classifier.
This is different to regular multi-class classification where one prediction is made from a distribution over $k$ classes and $\log_2(k) \leq b \leq k$.
\fi

\iffalse
At this point, we highlight that ECOC is distinctly different to other typical multi-label approaches, such as 1-vs-rest or 1-vs-1 multi-classification. The former attempts to distinguish a single class from the rest and repeat for all classes, treating the problems as multiple binary classifications. The latter \textbf{finish}
\fi



\iffalse
~\citep{ferng2011multi} have also extended ECOC to multi-label classification. They also show that performance can be further improved by adding more parity bits for error-checking, trading-off the amount of bits depending the difficulty of the task. In this work, we too test varying amount of error-correcting codes and compare against the minimal amount that are needed. 
\fi

==> notes/conc.tex <==
% right before conclusion 
\iffalse
for when ordering latent tree and ecoc via word embedding similarity, as defined by the $\mathtt{skipgram}$ algorithms

We now compare how mixture sampling compares alternative methods that also look to mitigate compounding errors. 

In contrast, there is no direct analogy of scheduled sampling which would be the equivalent of interpolating between the dimensions of the predicted conditional distribution and the target (which has all point mass on a single discrete token and 0 everywhere else). 
\fi

% in conclusion

\iffalse
This work has introduced a latent variable neural language model based on error-correcting output codes as the main contribution. From this, we propose many novel methods for using such networks to approximate the conditional and propose the first method that mitigates exposure bias for latent-models. We demonstrate these new techniques in the context of the proposed error-correcting neural language model.
\fi

\iffalse This involved sampling from the model distribution according to predict codewords throughout training. \fi

==> notes/ensemble_mix_methods.tex <==
\iffalse
\subsection{Ensemble Mixture Methods}
% http://proceedings.mlr.press/v48/lij16.pdf

For cases where computational resources and speed are not a concern, some work has looked at ensemble-based language modelling. Ensemble learning has shown superior performance in general machine learning. This work is distinctly different to other work in Equation \ref{sec:rr} since it involves using more memory but with the benefit of alleviating the information bottleneck in the decoder. Similarly, mixture models can also be viewed as a type of ensemble method with a mixture coefficient, akin to weighted averaging in ensembles. In the context of language modelling, this is equivalent to using Conditional Bernoulli Mixtures. These models have also been used in multi-label classification ~\citep{li2016conditional}, and can capture dependencies between labels while requiring less computation than comparable multi-label classification approaches. 
~\citep{yang2017breaking} formulate language modelling as matrix factorization and show that a single softmax can lead to low rank approximation, which compresses the input too much (i.e. bottleneck) for high dimensional problems such as language modelling. Their solution is to combine more than one softmax on the decoder layer. This approach led to large reduction in perplexity for PTB, WikiText-2 and 1-Billion word datasets.
\fi


\iffalse
In subsequent analysis, we will compare these approaches to using a mixture of ECOCs where error-correcting codes are designated $K$ mixtures.  
\fi

==> notes/evaluation.tex <==

\iffalse
\begin{equation}
     \mathcal{L}^{\text{ECOC}} = - \frac{1}{N}\sum_{i=1}^{N} y \log\Big(\prod_{c}^{C}\max_{k}\big(\phi(x, h_t)\big)\Big)
\end{equation}
\fi

\iffalse

\paragraph{Evaluating Mixture of ECOCs}
We compare ECOC latent-variable mixture model against hierarchical softmax mixtures (HSM),  of adaptive softmax mixtures (ASM) and full softmax mixtures (FSM). To ensure a fair comparison is carried out we assign the same number of unique codewords as there are classes in HSM and approximately the same number of weights for ECOC as in AS.

\subsection{Evaluation Measures}
Perplexity is the predominant evaluation measure in language modelling since a recurrent neural networks decodes from the hidden state vectors and produces a probability distribution using softmax normalization over all word in the vocabulary. 
In ECOC however, we do not predict the posterior in this way since the aim is to avoid having to compute the extra computation in performing a softmax operation. Therefore, we must consider an evaluation measure for ECOC, that is in some way comparable to models that produce posteriors. 

We chose to store codewords when modelling using standard cross-entropy for multi-class classification and convert the predicted token (via argmax operation) to codewords and compute the Hamming distance (analogous to word error rate in machine translation and speech recognition). We make sure that the codebooks are shared among both approaches, both when experimenting with random codeword assignment orders and re-orderings based on cosine similarity of word embeddings, or co-occurrence matrix row jaccard similarity. 

This is then directly comparable to our approach. Similarly, both methods are comparable for accuracy. 
\fi

==> notes/gumbel_softmax.tex <==
% after end of gumbel softmax paragraph 

\iffalse
Lastly, we define the gradient of the log-likelihood loss when using LVMS as Equation \ref{eq:cms_loss}. 


\begin{equation}\label{eq:cms_loss}
\begin{gathered}
 \frac{\partial}{\partial \theta} \mathbb{E}_{p(b)}[f(b)] \approx \mathbb{E}_{p(u)}\Big[\frac{\partial}{\partial \theta}f(\sigma_{\lambda}(z( \theta, u))\Big]
 \end{gathered}
\end{equation}
\fi


\iffalse
The objective can then be expressed as the following, 

\begin{equation}
    \mathcal{L}_{\theta} = 
\end{equation}

Consider an unnormalized parameterization (α1, . . . , αn) where αk ∈ (0, ∞) of a discrete distribution D ∼ Discrete(α)—we can assume that states with 0 probability are excluded. The GumbelMax trick proceeds as follows: sample Uk ∼ Uniform(0, 1) i.i.d. for each k, find k that maximizes
{log αk − log(− log Uk)}, set Dk = 1 and the remaining Di = 0 for i 6= k. Then P(Dk = 1) = P αk n_{i}=1 \alpha_i. (9) In other words, the sampling of a discrete random variable can be refactored into a deterministic
function—componentwise addition followed by argmax—of the parameters log αk and fixed distribution − log(− log Uk). See Figure 1a for a visualization.
\fi



\iffalse
We will use this `concrete' approximation of softmax sampling in our relaxation of scheduled sampling with a sample-based decoder. We discuss details in the next section. Note that our original motivation based on removing discontinuity does not strictly apply to this sampling procedure, which still yields a stochastic gradient due to sampling from the Gumbel distribution. However, this approach is conceptually related to greedy relaxations since, here, the soft argmax reparametrization reduces gradient variance which may yield a more informative training signal. Intuitively, this approach results in the gradient of the loss to be more aware of the sampling procedure compared to naive scheduled sampling and hence carries forward information about decisions made at previous steps. The empirical results, discussed later, show similar gains to the greedy scenario.
\fi

\iffalse
\section{Final Comments}
ECOC is a latent variable approach that directly maximizes the probability of the latent variable code (i.e. codeword), unlike all previous approaches that instead output probabilities over all possible outputs. The latter can include latent short codes (e.g hierarchical softmax), but only for the purpose of maximizing the log-likelihood at training the time, softmax normalization still needs to be used at test time to predict the next token. In contrast, this is not required for ECOC as the targets are the latent codes, which means the computational benefits are still found at test time. The benefit of using binary codes, as opposed to codes that contain more than 2 children along the tree (e.g octal, decimal or hexadecimal), is that binary latent codes allow us to avoid the cost of normalization since each codebit is minimized independently using a binary cross-entropy loss. For example, if each codebit represents hexadecimal, then it requires that we use a softmax to normalize the probabilities when using cross-entropy over for each codebit. Not to mention, that binary codes are still relatively short ($\log_2(\mathcal{V})$) even for a large vocabulary, and when using many error-correcting bits. That said, if one has enough memory then this can certainly be achieved in our framework.
\fi

\iffalse Given enough error-correcting bits such that the number of unique codewords \fi



\iffalse
We demonstrate two implementations of our method
using logistic regressions and gradient boosted
trees, together with a simple training procedure
based on Expectation Maximization. We further
derive an efficient prediction procedure based on
dynamic programming, thus avoiding the cost of
examining an exponential number of potential label
subsets. Experimental results show the effectiveness
of the proposed method against competitive
alternatives on benchmark datasets
\fi

==> notes/hsoftmax.tex <==
\iffalse
 A Huffman binary tree has been used in the past~\citep{mikolov2013distributed} to assign these codes, while others have proposed using a more semantic-based approach by using word relations from WordNet and forming a binary tree via clustering a tf-idf matrix ~\citep{morin2005hierarchical}.
This approach is the most relevant to our work, which we will discuss in Equation \ref{sec:pm_ecoc} 
\fi

==> notes/intro.tex <==
\iffalse the dimensionality of the output is proportional to the vocabulary size $|\mathcal{V}|$ and so\fi
 
\iffalse There has been methods for reducing the number of the parameters in the decoder by approximating the softmax~\citep{bengio2003neural,grave2016efficient,chen2015strategies}\fi \iffalse
There has been a plethora of methods for dealing with such problems, not only in language modelling~\citep{bengio2003neural} but also in distributed word representations ~\citep{mikolov2013distributed}\iffalse (we will discuss in Equation \ref{sec:rr})\fi.
\fi

\iffalse , reduce the output dimensionality to $\log_2(|\mathcal{V}|)$.  This time and memory reductions at both train and test time, at the expense of some accuracy. However, we show\fi


% before contributions

\iffalse
Moreover, we find the gumbell softmax trick and show that it outperforms an equivalent sampling method when using the predictive distributions in the defacto multi-classifcation language modelling setup. We begin by briefly introducing error codes and more recent applications of them in machine learning.
\fi

==> notes/latent_var_mix_samp.tex <==
\iffalse
\paragraph{Gumbel Mixture Sampling}
We also consider 

\subsection{Codeword Objective}
The loss function $\mathcal{L}_{\theta}(y_t, \hat{y}_t)$ is then given as Equation \ref{eq:bce}. 
\begin{equation}\label{eq:bce}
\sum_{i \in N} y_{t-1}^{i}\log(\hat{y}_{t-1}^{i}) + (1-y_{t-1}^{i})\log(1-\hat{y}_{t-1}^{i})
\end{equation}
\fi

\iffalse
\begin{figure}
    \includegraphics[scale=.7]{images/secoc.jpg}
    \caption{Error-Coded Language Model Mixture Sampling )}\label{fig:ppl_loss_surface}
\end{figure}
\fi

\iffalse
% didn't realize, but best results were with the sigmoid schedule
\begin{gather}\label{eq:cur_exp}
    p(\hat{y}_{t-1}=x_{t}) = 1 - \frac{\epsilon}{N}\exp(-\frac{\epsilon}{N}) \;, \forall \epsilon \in [0,1,..,N]
\end{gather}
\fi

==> notes/results.tex <==
\begin{table}
\resizebox{1.\linewidth}{!}{%
\begin{tabular}{c|cc|cc|cc}
\toprule[0.2em]
 & \multicolumn{2}{c}{\textbf{PTB}} &  \multicolumn{2}{c}{\textbf{WikiText-2}} &  \multicolumn{2}{c}{\textbf{WikiText-103}} \\

& Val. & Test & Val. & Test & Val. & Test\\

\midrule
SS-SM & 81.17 & 75.24 & 124.01 & 119.30 & 56.72 & 49.35 \\
Soft-SS-SM & \textbf{\emph{77.48}} & \textbf{\emph{69.81}} & \textbf{\emph{119.93}} & \textbf{\emph{115.27}} & \textbf{\emph{54.02}} & \textbf{\emph{45.77}} \\
SS-Adaptive-SM & 82.45 & 78.03 & 122.37 & 118.59 & 57.81 & 49.08 \\
SS-Hierarchical-SM & 85.56 & 78.17 & 123.88 & 120.91 & 59.76 & 51.59 \\
CLVMS-Hierarchical-SM & 84.11 & 77.13 & 123.23 & 121.35 & 59.56 & 50.41 \\
DLVMS-Hierarchical-SM & 81.83 & 77.40 & 123.51 & 121.78 & 58.63 & 52.72 \\
\midrule
SS-ECOC & 86.02 & 78.57 & 124.39 & 120.81 & 58.23 & 50.29 \\
Soft-SS-ECOC & 85.11 & 77.59 & 123.94 & 120.82 & 57.01 & 49.26 \\
\midrule[0.15em]

CLVMS-ECOC & 80.67 & 78.39 & \textbf{\emph{122.27}} & \textbf{\emph{117.90}} & \textbf{\emph{57.81}} & \textbf{\emph{50.03}} \\
DLVMS-ECOC & 79.67 & 76.39 & \textbf{\emph{119.27}} & \textbf{\emph{117.41}} & 59.35 & 51.67 \\

\bottomrule[0.2em]
\end{tabular}%
}
   \caption{\small{Perplexities for techniques that mitigate Exposure Bias}}\label{tab:ecoc_embedding_results} 
\end{table}

==> notes/sampling_based_methods.tex <==
\subsubsection{Sampling-Based Methods}
\iffalse
Sampling approaches instead approximate the normalization of the softmax (i.e. large sum of exponentials) by sampling only few elements in the output space. However, this only works during training, as the normalization still needs to be computed at test time.
\fi
\textbf{Importance Sampling} (IS) is a classical Monte-carlo sampling method used to approximate probability distributions. A proposal distribution $Q$ is used to approximate the true distribution $P$ which allows us to draw Monte-Carlo samples at much less cost than if we were to draw directly from $P$. $Q$ is often chosen to be simple and close to $P$. In language modelling, it is common that the unigram distribution is used for $Q$. \iffalse Equation \ref{eq:is_expectation} shows\fi The expectation $  \mathbb{E}_{w_i \sim P[\nabla_{\theta}\varphi(w_i)]} \approx \sum_{i=1}^{m}\nabla_{\theta}\varphi(w_i)$ over sampled word $w_i$ that is approximately the gradient of $\varphi(w_i)$.
\iffalse, like the aforementioned use of it for negative sampling.

\begin{equation}\label{eq:is_expectation}
    \mathbb{E}_{w_i \sim P[\nabla_{\theta}\varphi(w_i)]} \approx \sum_{i=1}^{m}\nabla_{\theta}\varphi(w_i)
\end{equation}
\fi
However, computing $p(w)$ for each sample is still required and therefore there have been methods to compute the product of marginals that avoids expensive normalization over the MC samples ~\citep{bengio2003neural}.
\iffalse
\textbf{Adaptive Importance Sampling} ~\citep{jean2014using} (AIS) only considers a set fraction of target tokens to sample from. This involves partitioning the training set where each partition is designated a subset of the vocabulary $V^{'} \subset V$. Therefore, there is a separate predictive distribution \iffalse(or should this be called proposal distribution $Q$)\fi for each partition and for a given partition $V^{'}$ all words within $V^{'}$ are assigned some probability.
\fi
\textbf{Noise Contrastive Estimation} ~\citep{mnih2012fast} propose to use Noise Contrastive Estimation (NCE)\iffalse ~\citep{gutmann2010noise}\fi as a sampling method in an unnormalized probabilistic model that is more stable than IS (can lead to diverging model distribution $Q$ in relation to underlying distribution $P$). Similar to our proposed ECOC-NLM, NCE treats density estimation as multiple binary classification problems, but is different in that it does so by discriminating between both data samples and a known noise distribution (e.g noise proportional to the unigram distribution). The posterior can be expressed in the context independent case as $P^{h}(D = 1|w, \theta) = P^h_{\theta}(w)/\big(P^h_{\theta}(w) + k P_n(w)\big)$ for hidden state $h$, parameterized by $\theta$ for $k$ generated samples. NCE is different from IS since it does not estimate the word probabilities directly, but instead uses an auxiliary loss that maximizes the probability of correct words from noisy samples. 



\iffalse
In the language modelling setting, the data distribution Phd(w) will be the distribution of words that occur after a particular context h. Though it is possible to use context-dependent noise distributions, for simplicity we will use a context-independent (unigram) Pn(w). We are interested in fitting the context-dependent
model Phθ(w) to Phd(w).

Noise Contrastive Estimation (NCE) (Gutmann and Hyvärinen, 2010) [14] is proposed by Mnih and Teh (2012) [15] as a more stable sampling method than Importance Sampling (IS), as we have seen that IS poses the risk of having the proposal distribution $Q$ diverge from the distribution $P$ that should be optimized. In contrast to the former, NCE does not try to estimate the probability of a word directly. Instead, it uses an auxiliary loss that also 
optimises the goal of maximizing the probability of correct words.

Recall the pairwise-ranking criterion of Collobert and Weston (2008) that ranks positive windows higher than "corrupted" windows, which we discussed in the previous post. NCE does a similar thing: We train a model to differentiate the target word from noise. We can thus reduce the problem of predicting the correct word to a binary classification task, where the model tries to distinguish positive, genuine data from noise samples, as can be seen in Figure 4 below.

\fi





\iffalse
\paragraph{Infrequent Normalization}
Andreas and Klein (2015) [21] suggest that it should even be sufficient to only normalise a fraction of the training examples and still obtain approximate self-normalising behaviour. They thus propose Infrequent Normalisation (IN), which down-samples the penalty term, making this a sampling-based approach.

Let us first decompose the sum of the previous loss $J_{\theta}$
 into two separate sums:
 
 \begin{equation}
     J_{\theta} = \sum_i h^{T}V^{'}_{w_i} + \alpha \sum_{i}\log^{2}(Z_c)
 \end{equation}

We can now down-sample the second term by only computing the normalisation for a subset $C$ of words $w_j$ and thus of contexts $c_j$ (as $Z(c)$ only depends on the context $c$) in the training data:

 \begin{equation}
     J_{\theta} = \sum_i h^{T}V^{'}_{w_i} + \frac{\alpha}{\gamma} \sum_{c_j \in C}\log^{2}(Z_{c_j})
 \end{equation}

\fi
